Symplectic birational transformations of finite order on O'Grady's sixfolds

We prove that any symplectic automorphism of finite order on a manifold of type OG6 acts trivially on the Beauville--Bogomolov--Fujiki lattice and that any birational transformation of finite order acts trivially on its discriminant group. Moreover, we classify all possible invariant and coinvariant sublattices.

==> tables/prime.sp.OG6.tex <==
%\begin{landscape}
\begin{center}
\begin{longtable}{lllllll}

 \caption{Coinvariant and invariant lattices for \(G \subset \Orth(\bL)\) of prime order with \(\bL_G\) negative definite (see \autoref{prop:table.OG6} and \autoref{thm:main.sp.OG6.old}).}
 \label{tab:prime.sp.OG6} \\
 
 \toprule
 No. & \(|G|\) & \(|G^\sharp|\) & \(\bL_G(-1)\) & \(\bL^G\) & example & \(\square\) \\ 
 \midrule
 \endfirsthead

 \multicolumn{6}{c}%
 {\tablename\ \thetable{}, follows from previous page} \\
 \midrule
 No. & \(|G|\) & \(|G^\sharp|\) & \(\bL_G(-1)\) & \(\bL^G\) & example & \(\square\) \\ 
 \midrule
 \endhead

 \midrule
 \multicolumn{6}{c}{Continues on next page} \\ 
 \endfoot

 \bottomrule
 \endlastfoot
 
 1 & \(2\) & \(1\) & \([2]\) & \(3\bU \oplus [-2]\) & {\tiny \(\begin{pmatrix} 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\spadesuit\) \\
 2 & \(2\) & \(1\) & \([2]\) & \(2\bU \oplus [2] \oplus 2[-2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
 3 & \(2\) & \(1\) & \(2[2]\) & \(3\bU\) & {\tiny \(\begin{pmatrix} 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \end{pmatrix}\)} & \(\spadesuit\clubsuit\) \\
 4 & \(2\) & \(1\) & \(2[2]\) & \(2\bU \oplus \bU(2)\) & {\tiny \(\begin{pmatrix} 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -1 & -2 \\ 0 & 0 & 0 & 0 & -2 & -2 & -2 & -1 \end{pmatrix}\)} & \(\clubsuit\) \\
 5 & \(2\) & \(1\) & \(2[2]\) & \(2\bU \oplus [2] \oplus [-2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\spadesuit\) \\
 4 & \(2\) & \(1\) & \(2[2]\) & \(\bU \oplus 2[2] \oplus 2[-2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
 5 & \(2\) & \(1\) & \(3[2]\) & \(2\bU \oplus [2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \end{pmatrix}\)} & \(\spadesuit\clubsuit\) \\
 6 & \(2\) & \(1\) & \(3[2]\) & \(\bU \oplus [2] \oplus \bU(2)\) & {\tiny \(\begin{pmatrix} 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -1 & -2 \\ 0 & 0 & 0 & 0 & -2 & -2 & -2 & -1 \end{pmatrix}\)} & \(\clubsuit\) \\
 7 & \(2\) & \(1\) & \(3[2]\) & \(\bU \oplus 2[2] \oplus [-2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\spadesuit\) \\
 8 & \(2\) & \(1\) & \(3[2]\) & \(3[2] \oplus 2[-2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
 9 & \(2\) & \(1\) & \(\bD_4\) & \(\bU \oplus 2[2]\) & {\tiny \(\begin{pmatrix} 3 & 4 & 2 & -2 & 0 & 0 & 2 & 2 \\ 4 & 3 & 2 & -2 & 0 & 0 & 2 & 2 \\ -2 & -2 & -1 & 2 & 0 & 0 & -1 & -1 \\ 2 & 2 & 2 & -1 & 0 & 0 & 1 & 1 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ -4 & -4 & -2 & 2 & 0 & 0 & -3 & -2 \\ -4 & -4 & -2 & 2 & 0 & 0 & -2 & -3 \end{pmatrix}\)} & \(\clubsuit\) \\
 10 & \(2\) & \(1\) & \(\bD_4\) & \(3[2] \oplus [-2] \) & {\tiny \(\begin{pmatrix} 3 & 4 & 2 & -2 & 2 & -2 & 2 & 0 \\ 4 & 3 & 2 & -2 & 2 & -2 & 2 & 0 \\ -2 & -2 & -1 & 2 & -1 & 1 & -1 & 0 \\ 2 & 2 & 2 & -1 & 1 & -1 & 1 & 0 \\ -2 & -2 & -1 & 1 & -1 & 2 & -1 & 0 \\ 2 & 2 & 1 & -1 & 2 & -1 & 1 & 0 \\ -4 & -4 & -2 & 2 & -2 & 2 & -3 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
 11 & \(2\) & \(1\) & \(4[2]\) & \(\bU \oplus 2[2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \end{pmatrix}\)} & \(\spadesuit\clubsuit\) \\
 12 & \(2\) & \(1\) & \(4[2]\) & \(2[2] \oplus \bU(2)\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -1 & -2 \\ 0 & 0 & 0 & 0 & -2 & -2 & -2 & -1 \end{pmatrix}\)} & \(\clubsuit\) \\
 13 & \(2\) & \(1\) & \(4[2]\) & \(3[2] \oplus [-2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\spadesuit\) \\
 14 & \(2\) & \(1\) & \(\bD_4 \oplus [2]\) & \(3[2]\) & {\tiny \(\begin{pmatrix} 3 & 4 & 2 & -2 & 2 & -2 & 2 & 0 \\ 4 & 3 & 2 & -2 & 2 & -2 & 2 & 0 \\ -2 & -2 & -1 & 2 & -1 & 1 & -1 & 0 \\ 2 & 2 & 2 & -1 & 1 & -1 & 1 & 0 \\ -2 & -2 & -1 & 1 & -1 & 2 & -1 & 0 \\ 2 & 2 & 1 & -1 & 2 & -1 & 1 & 0 \\ -4 & -4 & -2 & 2 & -2 & 2 & -3 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \end{pmatrix}\)} & \(\spadesuit\clubsuit\) \\
 15 & \(2\) & \(1\) & \(\bD_4 \oplus [2]\) & \(3[2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & -1 & 2 & -2 & -2 & -1 & -1 \\ 0 & 0 & 2 & -1 & 2 & 2 & 1 & 1 \\ 0 & 0 & 2 & -2 & 3 & 4 & 2 & 2 \\ 0 & 0 & 2 & -2 & 4 & 3 & 2 & 2 \\ 0 & 0 & -2 & 2 & -4 & -4 & -3 & -2 \\ 0 & 0 & -2 & 2 & -4 & -4 & -2 & -3 \end{pmatrix}\)} & \(\clubsuit\)  \\ % the vector (0,0, 0,0, 2,0, 1,1) has square -4 and divisibility 2
 16 & \(2\) & \(1\) & \(5[2]\) & \(3[2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \end{pmatrix}\)} & \(\spadesuit\clubsuit\) \\
 \midrule
 17 & \(2\) & \(2\) & \([4]\) & \(3\bU \oplus [-4]\) & {\tiny \(\begin{pmatrix} 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \end{pmatrix}\)} & \(\clubsuit\) \\
 18 & \(2\) & \(2\) & \([2] \oplus [4]\) & \(2\bU \oplus [-4] \oplus [2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \end{pmatrix}\)} & \(\clubsuit\) \\
 19 & \(2\) & \(2\) & \(\bA_3\) & \(2\bU \oplus [4]\) & {\tiny \(\begin{pmatrix} 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -2 & -1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -1 & -2 \end{pmatrix}\)} & \(\clubsuit\) \\
 20 & \(2\) & \(2\) & \(2[2] \oplus [4]\) & \(\bU \oplus [-4] \oplus 2[2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \end{pmatrix}\)} & \(\clubsuit\) \\
 21 & \(2\) & \(2\) & \(\bA_3 \oplus [2]\) & \(\bU \oplus [4] \oplus [2]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -2 & -1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -1 & -2 \end{pmatrix}\)} & \(\clubsuit\) \\
 22 & \(2\) & \(2\) & \(3[2] \oplus [4]\) & \(3[2] \oplus [-4]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \end{pmatrix}\)} & \(\clubsuit\) \\
 23 & \(2\) & \(2\)  & \(\bD_5\) & \(\bA_3\) & {\tiny \(\begin{pmatrix} 1 & 2 & 0 & 2 & 0 & 2 & 1 & 1 \\ 2 & 1 & 0 & 2 & 0 & 2 & 1 & 1 \\ 2 & 2 & 1 & 4 & 0 & 4 & 2 & 2 \\ 0 & 0 & 2 & 1 & 0 & 2 & 1 & 1 \\ 2 & 2 & 2 & 4 & 1 & 6 & 3 & 3 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ -2 & -2 & -2 & -4 & -2 & -6 & -4 & -3 \\ -2 & -2 & -2 & -4 & -2 & -6 & -3 & -4 \end{pmatrix}\)} & \(\clubsuit\) \\ 
 24 & \(2\) & \(2\) & \(\bA_3 \oplus 2[2]\) & \(2[2] \oplus [4]\) & {\tiny \(\begin{pmatrix} 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 \\ 0 & 0 & 0 & 0 & 2 & 1 & 1 & 1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -2 & -1 \\ 0 & 0 & 0 & 0 & -2 & -2 & -1 & -2 \end{pmatrix}\)} & \(\clubsuit\) \\ 
 \midrule
 25 & \(3\) & \(1\) & \(\bA_2\) & \(2\bU \oplus \oplus [6] \oplus [-2]\) & {\tiny \(\begin{pmatrix} 1 & 1 & 1 & -1 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ -1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
 26 & \(3\) & \(1\) & \(2\bA_2\) & \(\bU \oplus 2[6]\) & {\tiny \(\begin{pmatrix} 1 & 1 & 1 & -1 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ -1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\ 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 1 & 1 & 0 \\ 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & -2 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
 \midrule
 27 & \(5\) & \(1\) & \(\bA_4\) & \({\footnotesize \begin{pmatrix} 2 & 1 & 0 \\ 1 & 2 & 1 \\ 0 & 1 & 4 \end{pmatrix}} \oplus [-2]\) & {\tiny \(\begin{pmatrix} 1 & 1 & 1 & -1 & 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 1 & 1 & -1 & 0 & 0 \\ 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1 & 1 & 1 & 0 \\ 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 \\ -2 & 0 & -2 & 0 & -2 & 0 & -1 & 0 \\ 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \end{pmatrix}\)} & \(\diamondsuit\) \\
\end{longtable}
\end{center}
%\end{landscape}

